Efficient Sentiment Analysis: A Resource-Aware Evaluation of Feature Extraction Techniques, Ensembling, and Deep Learning Models

While reaching for NLP systems that maximize accuracy, other important metrics of system performance are often overlooked. Prior models are easily forgotten despite their possible suitability in settings where large computing resources are unavailable or relatively more costly. In this paper, we perform a broad comparative evaluation of document-level sentiment analysis models with a focus on resource costs that are important for the feasibility of model deployment and general climate consciousness. Our experiments consider different feature extraction techniques, the effect of ensembling, task-specific deep learning modeling, and domain-independent large language models (LLMs). We find that while a fine-tuned LLM achieves the best accuracy, some alternate configurations provide huge (up to 24, 283 *) resource savings for a marginal (<1%) loss in accuracy. Furthermore, we find that for smaller datasets, the differences in accuracy shrink while the difference in resource consumption grows further.

==> extra.tex <==
\begin{table*} [!thbp]
\begin{center}
{\small
\begin{tabular}{ |l|l|l|l|l|l|l|l|  }
\hline
\multicolumn{8}{ |c| }{IMDB Review Dataset} \\

\hline
Feature Extraction Method & Classifier & Accuracy & RMSE & Time & Memory & Energy & CO$_2$ \\ \hline 

\multirow{3}{*}{BOW} & SVM & 87.86 & 34.84 & 18.75 & 178.72 & 3.66 & 1.701\\
 & Voting & 88.06 & 34.55 & 82.01 & 181.61 & 16.02 & 7.442\\
 & Boosting & 85.40 & 38.20 & 0.16 & 152.82 & 0.03 & 0.015 \\ \hline
 \multirow{3}{*}{TF-IDF} & SVM & \textbf{90.11} & 31.44 & 22.87 & 179.36 & 4.46 & 2.075 \\
 & Voting & 89.82 & 31.84 & 103.93 & 182.28 & 20.30 & 9.432\gknote{Do we know why this one cost so much more?} \\
 & Boosting & 85.56 & 38.00 & 0.22 & 154.21 & 0.04 & 0.020 \\ \hline
\multirow{3}{*}{CBOW} & SVM & 61.43 & 62.10 & 3.60 & 106.41 & 0.70 & 0.327 \\
 & Voting & 61.26 & 62.24 & 10.29 & 106.36 & 2.011 & 0.934 \\
 & Boosting & 60.10 & 63.16 & 2.12 & 79.07 & 0.41 & 0.192\\ \hline
\multirow{3}{*}{FastText} & SVM & 88.64 & 33.70 & 0.34 & 65.58 & 0.06 & 0.031 \\
 & Voting & 81.25 & 43.30 & 2.38 & 66.06 & 0.46 & 0.216 \\
 & Boosting & 88.40 & 34.05 & 0.08 & 60.69 & 0.017 & 0.0076 \\ \hline
\multirow{3}{*}{DWE} & SVM & 88.72 & 33.58 & 5.24 & 745.46 & 1.02 & 0.476 \\
 & Voting & 86.47 & 36.78 & 11.22 & 732.16 & 2.19 & 1.018 \\
 & Boosting & 88.73 & 33.58 & 3.25 & 710.59 & 0.63 & 0.295 \\ \hline
\multirow{3}{*}{CNN} & SVM & 89.59 & 32.26 & 89.82 & 6519.82 & 17.54 & 8.151\\
 & Voting & 89.65 & 32.17 & 337.81 & 6519.87 & 65.98 & 30.655 \\
 & Boosting & 88.63 & 33.71 & 11.16 & 5150.24 & 2.81 & 1.013 \\ \hline
\multirow{3}{*}{LSTM} & SVM & 88.62 & 33.73 & 123.10 & 361.67 & 24.04 & 11.172 \\
 & Voting & 88.37 & 34.10 & 126.95 & 362.14 & 24.80 & 11.521 \\
 & Boosting & 87.87 & 34.82 & 122.45 & 355.43 & 23.92 & 11.112\\ \hline
\multirow{3}{*}{RoBERTa-base} & SVM & 83.88 & 40.14 & 51.93 & 774.55 & 10.14 & 4.712 \\
 & Voting & 85.78 & 37.70 & 70.76 & 732.08 & 6.87 & 3.194 \\
 & Boosting & 84.60 & 39.24 & 43.44 & 632.45 & 8.48 & 3.941 \\ \hline
 \multirow{3}{*}{RoBERTa-base+FastText} & SVM & 89.51 & 32.43 & 48.85 & 747.90 & 9.543 & 4.433 \\
 & Voting & 89.27 & 32.75 & 63.06 & 747.43 & 12.32 & 5.723 \\
 & Boosting & 88.94 & 33.12 & 45.80 & 691.29 & 8.943 & 4.156 \\ \hline 
\hline

 \multicolumn{2}{| c |}{\textit{Standalone RoBERTa Baseline}} & \textbf {91.02} & 30.44 & 997.88 & 606.14 & 201.05 & 90.554 \\ \hline
\end{tabular}
}
\end{center}
\caption{\label{tab:IMDB-tests}Results of IMDB review dataset on different feature extraction method}
\end{table*}


\begin{table*} [!htbp]
%\setlength{\tabcolsep}{4.5pt}
\begin{center}
{\small
\begin{tabular}{ |l|l|l|l|l|l|l|l|  }
\hline
\multicolumn{8}{ |c| }{Restaurant Review Dataset} \\
\hline
Feature Extraction Method & Classifier & Accuracy & RMSE & Time & Memory & Energy & CO$_2$ \\ \hline
\multirow{3}{*}{BOW} & SVM & 94.51 & 23.41 & 0.04 & 6.74 & 0.008 & 0.003\\
 & Voting & 95.76 & 20.56 & 0.23 & 7.24 & 0.046 & 0.021\\
 & Boosting & 94.80 & 22.78 & 0.008 & 6.10 & 0.002 & 0.0007 \\ \hline
 \multirow{3}{*}{TF-IDF} & SVM & 95.62 & 20.91 & 0.04 & 6.90 & 0.009 & 0.004 \\
 & Voting & 95.81 & 20.45 & 0.24 & 7.39 & 0.048 & 0.022 \\
 & Boosting & 94.56 & 23.30 & 0.008 & 6.29 & 0.002 & 0.0007 \\ \hline
\multirow{3}{*}{CBOW} & SVM & 77.88 & 47.02 & 0.078 & 12.69 & 0.015 & 0.007 \\
 & Voting & 78.75 & 46.09 & 0.34 & 12.92 & 0.068 & 0.031 \\
 & Boosting & 80.33 & 44.34 & 0.052 & 10.04 & 0.012 & 0.005\\ \hline
\multirow{3}{*}{FastText} & SVM & 96.01 & 19.97 & 0.007 & 6.41 & 0.001 & 0.0006 \\
 & Voting & 62.11 & 61.55 & 0.101 & 6.77 & 0.020 & 0.009 \\
 & Boosting & 95.91 & 20.21 & 0.011 & 6.18 & 0.002 & 0.001 \\ \hline
\multirow{3}{*}{DWE} & SVM &  96.10 & 19.73 & 2.05 & 553.84 & 0.402 & 0.186 \\
 & Voting & 63.79 & 60.16 & 2.25 & 552.60 & 0.442 & 0.205 \\
 & Boosting & 95.86 & 20.33 & 2.00 & 550.33 & 0.393 & 0.182 \\ \hline
\multirow{3}{*}{CNN} & SVM & 95.91 & 20.21 & 3.94 & 2948.43 & 0.770 & 0.35\\
 & Voting & 95.48 & 21.25 & 12.86 & 2933.23 & 2.51 & 1.167 \\
 & Boosting & 94.32 & 23.81 & 3.58 & 2641.68 & 0.70 & 0.325 \\ \hline
\multirow{3}{*}{LSTM} & SVM & 95.43 & 21.37 & 14.47 & 62.16 & 2.82 & 1.313 \\
 & Voting & 93.36 & 25.75 & 6.29 & 62.64 & 1.22 & 0.570 \\
 & Boosting & 95.14 & 22.03 & 14.93 & 62.07 & 2.91 & 1.355\\ \hline
\multirow{3}{*}{RoBERTa-base} & SVM & 80.24 & 44.45 & 5.36 & 149.62 & 1.048 & 0.486 \\
 & Voting & 92.30 & 27.73 & 5.03 & 149.30 & 0.489 & 0.227 \\
 & Boosting & 93.84 & 24.80 & 4.90 & 130.15 & 0.957 & 0.444 \\ \hline
 \multirow{3}{*}{RoBERTa-base+FastText} & SVM & \textbf{96.53} & 18.60 & 4.72 & 151.01 & 0.922 & 0.428 \\
 & Voting & 96.25 & 19.36 & 5.19 & 150.92 & 1.016 & 0.471 \\
 & Boosting & 95.81 & 20.45 & 4.69 & 142.47 & 0.917 & 0.425 \\ \hline
\hline

 \multicolumn{2}{| c |}{\textit{Standalone RoBERTa Baseline}} & \textbf {96.69} & 19.12 & 160.61 & 77.94 & 31.36 & 14.570  \\ \hline
\end{tabular}
}
\end{center}
\caption{\label{tab:restaurant-tests} Results of resturant review dataset on different feature extraction methods}
\end{table*}


\begin{table*} [!htbp]
\begin{center}
{\small
\begin{tabular}{ |l|l|l|l|r|l|l|l|  }
\hline
\multicolumn{8}{ |c| }{Product Review Dataset} \\
\hline
Feature Extraction Method & Classifier & Accuracy & RMSE & Time & Memory & Energy & CO$_2$ \\ \hline
\multirow{3}{*}{BOW} & SVM & 91.29 & 29.50 & 0.078 & 9.75 & 0.015 & 0.007\\
 & Voting & 91.29 & 29.50 & 0.392 & 10.27 & 0.077 & 0.035\\
 & Boosting & 91.05 & 29.90 & 0.012 & 8.59 & 0.002 & 0.001 \\ \hline
 \multirow{3}{*}{TF-IDF} & SVM & 92.83 & 26.76 & 0.081 & 9.90 & 0.016 & 0.007 \\
 & Voting & 92.08 & 28.12 & 0.403 & 10.41 & 0.079 & 0.036 \\
 & Boosting & 91.57 & 29.02 & 0.012 & 8.79 & 0.003 & 0.001 \\ \hline
\multirow{3}{*}{CBOW} & SVM & 75.88 & 49.10 & 0.120 & 14.83 & 0.023 & 0.010 \\
 & Voting & 78.79 & 46.05 & 0.432 & 14.89 & 0.085 & 0.039 \\
 & Boosting & 80.33 & 44.10 & 0.094 & 10.78 & 0.018 & 0.008\\ \hline
\multirow{3}{*}{FastText} & SVM & 93.44 & 25.60 & 0.010 & 7.33 & 0.002 & 0.001 \\
 & Voting & 90.73 & 30.44 & 0.136 & 7.63 & 0.027 & 0.012 \\
 & Boosting & 93.39 & 25.69 & 0.014 & 6.82 & 0.003 & 0.001 \\ \hline
\multirow{3}{*}{DWE} & SVM & 92.93 & 26.58 & 2.092 & 557.20 & 0.409 & 0.189 \\
 & Voting & 90.91 & 30.13 & 2.346 & 554.76 & 0.459 & 0.213 \\
 & Boosting &  93.82 & 24.85 & 2.070 & 551.72 & 0.405 & 0.188 \\ \hline
\multirow{3}{*}{CNN} & SVM & 92.32 & 27.70 & 5.430 & 3174.55 & 1.061 & 0.49\\
 & Voting & 92.04 & 28.21 & 19.801 & 3174.30 & 3.868 & 1.796 \\
 & Boosting & 91.47 & 29.19 & 3.648 & 2714.406 & 0.71 & 0.330 \\ \hline
\multirow{3}{*}{LSTM} & SVM & 91.43 & 29.27 & 14.787 & 64.78 & 2.889 & 1.342 \\
 & Voting & 92.83 & 26.76 & 6.403 & 65.49 & 1.251 & 0.581 \\
 & Boosting & 92.60 & 27.19 & 15.026 & 64.69 & 2.935 & 1.363\\ \hline
\multirow{3}{*}{RoBERTa-base} & SVM & 84.64 & 39.18 & 6.040 & 166.12 & 1.180 & 0.547 \\
 & Voting & 87.68 & 35.08 & 6.604 & 151.27 & 1.270 & 0.599 \\
 & Boosting & 90.26 & 31.20 & 5.528 & 133.97 & 1.080 & 0.501 \\ \hline
 \multirow{3}{*}{RoBERTa-base+FastText} 
 & SVM      & \textbf{93.94}    & 24.61     & 5.340     & 156.73    & 1.044     & 0.484 \\
 & Voting   & 93.35             & 25.78     & 6.150     & 156.28    & 1.202     & 0.558 \\
 & Boosting & 93.91             & 24.67     & 6.130     & 146.62    & 1.199     & 0.557 \\ \hline
 \hline

  \multicolumn{2}{| c |}{\textit{Standalone RoBERTa Baseline}} & \textbf {94.66} & 22.52 & 213.96 & 95.89 & 41.77 & 19.409  \\ \hline
\end{tabular}
}
\end{center}
\caption{\label{tab:product-tests}Results of product review dataset on different feature extraction methods} 
\end{table*}



\section{Related Work}
\todo{Add a high-level paragraph describing the general state of prior work before diving into details of specific systems.}
\todo[color=blue]{Take a note that this work will be available at github}.

Previous studies in sentiment analysis have investigated a wide range of methodologies, including traditional and deep machine learning models (particularly CNNs and RNNs) , as well as different feature extraction strategies. Many research studies have used well-known feature extraction techniques, such as BOW, TF-IDF, and N-Grams for sentiment analysis. Other studies have utilized widely-used pre-trained word embedding like FastText, GloVe, and word2vec  for creating input vectors.  Also, some research has employed transformer-based model in order to identify which is most effective at conducting sentiment analysis. 

\citet{zhou2022text} proposed a model that uses the double word embedding (DWE) method for sentiment classification. In their experiment, they used GloVe and word2vec to create a combinational input. For the structure of their dual-channel word embedding, they have used three different combinations of word2vec and GloVe. 

\citet{AHUJA2019341} considered the SS-Tweet dataset for sentiment
classification and used six different classifier models for analyzing the results. They have used two feature extraction techniques namely TF-IDF and N-Grams. According to their results, TF-IDF performed better than N-Grams. They also found that logistic regression gave the highest accuracy, precision, recall, and f1-score for both the TF-IDF and N-Gram feature extraction methods. They conducted their experiment by applying KNN, Decision Tree, SVM, Random Forest, Logistic Regression and Na{\"i}ve Bayes algorithms. 

\citet{alharbi2021evaluation} used three different feature extraction methods (i.e., GloVe, word2vec and FastText ) with simple RNN and it's four variants to perform sentiment analysis on Amazon product review. In their experiment they found that FastText worked better in most cases with different RNNs in terms of accuracy. They also showed their work for balanced and unbalanced data analysis for different RNN models. 

\citet{pranesh-shekhar-2020-analysis} performed comparative analysis of resource efficient ML models for four different text classification task. They have used 8 different machine learning models and evaluated these models in terms of accuracy and memory usage. Based on their experiment, they reached to the conclusion that Bonsai model performed well in most cases in terms of accuracy and memory usage. 

\citet{8876896} conducted a study where they investigated various deep learning techniques for analyzing Twitter data.  Particularly, they experimented with different combinations of convolutional neural networks (CNN) and recurrent neural networks (RNN), utilizing both GloVe and word2Vec word embeddings. They proposed a technique that combined multiple CNNs with bi-LSTM networks and GloVe embedding, and it outperformed all other tested techniques in terms of accuracy.
